Combining No-regret and Q-learning

Counterfactual Regret Minimization (CFR) has found success in settings like poker which have both terminal states and perfect recall. We seek to understand how to relax these requirements. As a first step, we introduce a simple algorithm, local no-regret learning (LONR), which uses a Q-learning-like update rule to allow learning without terminal states or perfect recall. We prove its convergence for the basic case of MDPs (and limited extensions of them) and present empirical results showing that it achieves last iterate convergence in a number of settings, most notably NoSDE games, a class of Markov games specifically designed to be challenging to learn where no prior algorithm is known to achieve convergence to a stationary equilibrium even on average.

==> cut.tex <==
This material cut because it is buggy.

\subsection{State and action independent $P$}

Another interesting special case is where $P_k(s' ~|~ s,a) = P_k(s' ~|~ s'',a'')$ for all $s$, $a$, $s'$, $s''$, and $a''$.  Thus we can instead write simply $P_k(s')$.  This case includes captures a version of the contextual banding problem where feedback is available about all actions rather than just the chosen one.

As in the previous special case, the operator is not constant over time but instead 
\begin{equation}
 \mathcal{T}_k Q(s,a) = \underbar{r}_k(s,a) + \gamma\mathbb{E}_{\underline{P}_k} [\max_i Q(s',a_i)],
\end{equation}
where $\underline{P}_k = \frac{1}{k} \sum_{k' = 0}^{k-1} P_{k'}$.
To prove a version of Lemma~\ref{lem:regret} for this setting we additionally need to change the way we report rewards to the no-regret algorithm.  The new update rule is
$x^s_{k,i} = P_k(s)Q_k(s,a_i)$.


\begin{lemma}
\begin{equation}
- \gamma |\mathcal{S}| \rho_{k-1}+  \mathcal{T}_k\underline{Q}_k(s,a) \leq\overline{Q}_k(s,a) \leq  \gamma |\mathcal{S}| \rho_{k-1}+  \mathcal{T}_k\underline{Q}_k(s,a).
\end{equation}
\end{lemma}
\begin{proof}
\begin{align*}
\overline{Q}_k(s,a)
&=  \frac{1}{k} \sum_{k' = 1}^k Q_{k'}(s,a)\\
&=  \frac{1}{k} \sum_{k' = 0}^{k-1} r_{k'}(s,a) + \gamma\mathbb{E}_{P_{k'},\pi_{k'}}[ Q_{k'}(s',a')]\\
&=  \frac{1}{k} \sum_{k' = 0}^{k-1} r_{k'}(s,a) +\gamma \sum_{s'} \frac{1}{k} \sum_{k' = 0}^{k-1}\mathbb{E}_{\pi_{k'}} [P_{k'}(s')Q_{k'}(s',a')]\\
&\geq \frac{1}{k} \sum_{k' = 0}^{k-1} r_{k'}(s,a)+ \gamma \sum_{s'} \max_i \frac{1}{k} \sum_{k' = 0}^{k-1}P_{k'}(s')Q_{k'}(s',a_i) - \rho_{k-1}\\
&= - \gamma |\mathcal{S}|\rho_{k-1} + \frac{1}{k} \sum_{k' = 0}^{k-1} r_{k'}(s,a)+ \gamma \sum_{s'} \max_i \frac{1}{k} \sum_{k' = 0}^{k-1}P_{k'}(s')Q_{k'}(s',a_i)\\
&= - \gamma |\mathcal{S}| \rho_{k-1} + \underbar{r}_k(s,a) + \gamma\mathbb{E}_{\underline{P}_k} [\max_i \underline{Q}_k(s',a_i)]\\
&= - \gamma |\mathcal{S}| \rho_{k-1}+  \mathcal{T}_k\underline{Q}_k(s,a)\\
\end{align*}
Again, we apply the no-regret property to obtain the inequality and the no-absolute-regret property to obtain the reverse inequality.
\end{proof}

Note how the weighting of the inputs to the no-regret algorithm is crucial to be able to apply the no-regret property in the proof.  Note also that the bounds we get here are worse than the previous versions by a $|\mathcal{S}|$ factor, although this may be an artifact of this particular proof.
